TimeCrypt: Encrypted Data Stream Processing at Scale with Cryptographic Access Control

A growing number of devices and services collect detailed time series data that is stored in the cloud. Protecting the confidentiality of this vast and continuously generated data is an acute need for many applications in this space. At the same time, we must preserve the utility of this data by enabling authorized services to securely and selectively access and run analytics. This paper presents TimeCrypt, a system that provides scalable and real-time analytics over large volumes of encrypted time series data. TimeCrypt allows users to define expressive data access and privacy policies and enforces it cryptographically via encryption. In TimeCrypt, data is encrypted end-to-end, and authorized parties can only decrypt and verify queries within their authorized access scope. Our evaluation of TimeCrypt shows that its memory overhead and performance are competitive and close to operating on data in the clear.

==> sections/discussion.tex <==
% !TEX root = ../paper_secure_TS.tex
	%\vspace{-0.5em}
\section{Discussion and Limitations}
\lsec{discussion}
	%\vspace{-0.5em}
	
\todo{I prefer that we move this text to the relevant places the first fot section 4.5 and the second to the evaluation section. I feel that this is becoming an easy material for lazy reviews to stuck. Maybe putting them whining the relevant context makes it harder for lazy reviewers.}	
%\oursystem enables a data management system to process statistical queries over encrypted time series data.
%At the same time, multiple principals can privately and efficiently query parts of the index they are authorized to access, while preserving data confidentiality.
We highlight some research questions that remain open.

\fakeparagraph{Richer statistics.}
\oursystem is optimized for  statistical range queries on encrypted time series data, the most common queries over such data (\rsec{background}).
Analyzing raw streams in their entirety is generally impractical if not infeasible~\cite{bailis2017macrobase}.
\oursystem provides powerful tools to search and retrieve relevant segments of the stream that can then be subject to  
advanced client-side processing after decryption.
Data mining and advanced queries, e.g., series similarity, distance measures, predictions, and pattern detection are currently not supported on encrypted data.
These are naturally more complex to process, and require specialized data structures and algorithms to be performed efficiently over big data~\cite{Faloutsos}.
%Moreover, this work focuses on intra-stream processing and does not address processing of queries across a collection of encrypted streams (i.e., inter-stream). --> we do


\fakeparagraph{Performance.}
\oursystem's encryption scheme consists of the key management that delivers one-time keys.
Our encryption is optimized for continuous aggregation segments and suffers from alternative patterns, such as aggregating 
every second data chunk.
Here the decryption overhead grows linearly with the number of aggregations and is not bound by a constant factor.
%For instance, a hash tree with $2^{30}$ keys induces a decryption overhead of 5.08~$\mu$s per aggregated value and amounts to 5.08~s for the decryption of 1~million non-continuous aggregations.


\begin{comment}
\fakeparagraph{Proof of computations \& range.}
The cloud can cheat with the computation, and a wrong range of a simple ciphertext may clutter the entire aggregated result.
\todo{Discuss two technical solutions which would allow these proofs, but would render the computation time too large!}
\end{comment}
